MegaSR: Mining Customized Semantics and Expressive Guidance for Real-World Image Super-Resolution

Text-to-image (T2I) models have ushered in a new era of real-world image super-resolution (Real-ISR) due to their rich internal implicit knowledge for multimodal learning. Although bringing high-level semantic priors and dense pixel guidance have led to advances in reconstruction, we identified several critical phenomena by analyzing the behavior of existing T2I-based Real-ISR methods: (1) Fine detail deficiency, which ultimately leads to incorrect reconstruction in local regions. (2) Block-wise semantic inconsistency, which results in distracted semantic interpretations across U-Net blocks. (3) Edge ambiguity, which causes noticeable structural degradation. Building upon these observations, we first introduce MegaSR, which enhances the T2I-based Real-ISR models with fine-grained customized semantics and expressive guidance to unlock semantically rich and structurally consistent reconstruction. Then, we propose the Customized Semantics Module (CSM) to supplement fine-grained semantics from the image modality and regulate the semantic fusion between multi-level knowledge to realize customization for different U-Net blocks. Besides the semantic adaptation, we identify expressive multimodal signals through pair-wise comparisons and introduce the Multimodal Signal Fusion Module (MSFM) to aggregate them for structurally consistent reconstruction. Extensive experiments on real-world and synthetic datasets demonstrate the superiority of the method. Notably, it not only achieves state-of-the-art performance on quality-driven metrics but also remains competitive on fidelity-focused metrics, striking a balance between perceptual realism and faithful content reconstruction.

==> parts/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/xinruili.jpg}}]{Xinrui Li}
received the B.Eng. degree from Shandong University, China, in 2024. He is currently pursuing the M.S. degree in Computer Science and Technology at the Harbin Institute of Technology (Shenzhen). His research interests include computer vision and visual content generation.
\end{IEEEbiography}
\vspace{-3em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/jinrongzhang.jpg}}]{Jinrong Zhang}
received the B.Eng. degree from Dalian University of Technology, China, in 2022, and the M.Eng. degree from Dalian University of Technology, China, in 2025. He is currently pursuing the Ph.D. degree with the School of Computer Science and Technology, Harbin Institute of Technology (Shenzhen), China. He has published papers in several top journals and conferences, including IEEE TNNLS, CVPR, AAAI, ACM MM, and ICME. His research interests include computer vision and multimodal learning.
\end{IEEEbiography}
\vspace{-3em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/jianlongwu.png}}]{Jianlong Wu}
(Member, IEEE) received the B.Eng. degree from the Huazhong University of Science and Technology, China, in 2014, and the Ph.D. degree from Peking University, China, in 2019. He is currently a Professor with the Harbin Institute of Technology (Shenzhen), China. He has published over 40 papers in top journals and conferences, such as IEEE TPAMI, ICML, NeurIPS, and ICCV. His research interests include computer vision and multimodal learning. He received many awards, such as the Outstanding Reviewer of ICML 2020 and the Best Student Paper of SIGIR 2021. He serves as the Associate Editor of IEEE TMM and IEEE TPAMI, and the Area Chair of  ICML, NeurIPS, CVPR, and ACM MM. 
\end{IEEEbiography}
\vspace{-2em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/chongchen.jpg}}]{Chong Chen}
received the B.S. degree in mathematics and the Ph.D. degree in statistics, under the supervision of Prof. Ruibin Xi from Peking University, Beijing, China, in 2013 and 2019, respectively. His research interests include image understanding, self-supervised learning, and data mining.
\end{IEEEbiography}
\vspace{-1em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/liqiangnie.jpg}}]{Liqiang Nie}
(Senior Member, IEEE) received the B.Eng. and Ph.D. degree from Xi’an Jiaotong University and National University of Singapore (NUS), respectively. After Ph.D., he continued his research in NUS as a research fellow for three years. He is currently the dean of the Department of Computer Science and Technology, Harbin Institute of Technology (Shenzhen). His research interests lie primarily in multimedia computing and information retrieval. He has co-/authored more than 150 papers and 5 books, with 34,000 plus Google Scholar citations. He is an AE of IEEE TIP, IEEE TKDE, IEEE TMM, IEEE TCSVT, ACM ToMM, and Information Science. Meanwhile, he serves as the chair of ICMR 2025, ICME 2025, and ACM MM 2027. He is a member of ICME steering committee. He has received many awards over the past four years, like SIGMM rising star in 2020, MIT TR35 China 2020, SIGIR best student paper in 2021, IEEE AI’s 10 to Watch in 2022, ACM MM Best paper award in 2022, and the National Youth Science and Technology Award in 2024.
\end{IEEEbiography}
%\vspace{-1em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/zhouchenlin.png}}]{Zhouchen Lin}
(Fellow, IEEE) received the Ph.D. degree in applied mathematics from Peking University in 2000. He is currently a Boya Special Professor with the State Key Laboratory of General Artificial Intelligence, School of Intelligence Science and Technology, Peking University.
His research interests include computer vision, image processing, machine learning, pattern recognition, and numerical optimization. He is a Fellow of IAPR, IEEE, AAIA and CSIG.
\end{IEEEbiography}
\vspace{-13mm}


==> tables/ft_datasets.tex <==
\begin{table}[t]
    \renewcommand\arraystretch{1.5}
    \caption{
    The quantitative evaluation of width-specific semantic requirements in T2I models.
    }
    \label{tab:ft_datasets}
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ccc}
            \hline
            Type & Model & Datasets \\
            \hline
            HED boundaries & HED & LSDIR \& DF2K \& FFHQ \\
            Depth maps & DepthAnythingV2 & LSDIR \& DF2K \& NYU\_depth\_v2 \\
            Segmentation masks & MaskDINO & LSDIR \& DF2K \& FFHQ \\
            CLIPV & CLIP & ImageNet-1k \\
            \hline
        \end{tabular}
    }
\end{table}

